NUNet: Deep Learning for Non-Uniform Super-Resolution of Turbulent Flows

Deep Learning (DL) algorithms are becoming increasingly popular for the reconstruction of high-resolution turbulent flows (aka super-resolution). However, current DL approaches perform spatially uniform super-resolution - a key performance limiter for scalability of DL-based surrogates for Computational Fluid Dynamics (CFD). To address the above challenge, we introduce NUNet, a deep learning-based adaptive mesh refinement (AMR) framework for non-uniform super-resolution of turbulent flows. NUNet divides the input low-resolution flow field into patches, scores each patch, and predicts their target resolution. As a result, it outputs a spatially non-uniform flow field, adaptively refining regions of the fluid domain to achieve the target accuracy. We train NUNet with Reynolds-Averaged Navier-Stokes (RANS) solutions from three different canonical flows, namely turbulent channel flow, flat plate, and flow around ellipses. NUNet shows remarkable discerning properties, refining areas with complex flow features, such as near-wall domains and the wake region in flow around solid bodies, while leaving areas with smooth variations (such as the freestream) in the low-precision range. Hence, NUNet demonstrates an excellent qualitative and quantitative alignment with the traditional OpenFOAM AMR solver. Moreover, it reaches the same convergence guarantees as the AMR solver while accelerating it by 3.2-5.5x, including unseen-during-training geometries and boundary conditions, demonstrating its generalization capacities. Due to NUNet's ability to super-resolve only regions of interest, it predicts the same target 1024x1024 spatial resolution 7-28.5x faster than state-of-the-art DL methods and reduces the memory usage by 4.4-7.65x, showcasing improved scalability.

==> text/background.tex <==
\section{Background}
\label{sec:background}

We use low-resolution steady incompressible
RANS problems for our non-uniform super-resolution task.
The RANS governing equations describe the motion 
of turbulent flows as follows: 

\vspace{-1em}
\begin{align}
  \frac{\partial \bar{U}_i}{\partial x_i} &= 0\label{eq:continuity}\\ \bar{U}_j
  \frac{\partial \bar{U}_i}{\partial x_j} &= \frac{\partial}{\partial
  x_j}\left[ -\left(\bar{p}\right)\delta_{ij}
  +\left(\nu+\nu_t\right)\left(\frac{\partial \bar{U}_i}{\partial x_j}
  + \frac{\partial \bar{U}_j}{\partial x_i}\right)\right]\label{eq:momentum}
\end{align} 

$\bar{U}$ is the mean velocity,
$\bar{p}$ is the kinematic mean pressure, $\nu$ is the fluid
laminar viscosity, and $\nu_t$ is the eddy viscosity. Equation~\ref{eq:momentum}
is a vector equation, hence it yields two scalar equations,
one for the first spatial direction and another for the second spatial direction. 

The RANS equations are a time-averaged solution to the incompressible Navier-Stokes equations but
result in a non-closed equation. We close the equation with Boussinesq's
approximation~\cite{boussinesq}. Boussinesq's approximation yields the eddy viscosity, 
which is found via modeling. 
A successful model, The Spalart-Allmaras one-equation model, is shown below and provides
a transport equation to compute the modified eddy viscosity, $\tilde{\nu}$.

\begin{multline}
\bar{U}_i \frac{\partial \tilde{\nu}}{\partial x_i } = C_{b1} \left(1-f_{t2}\right) \tilde{S} \tilde{\nu} - \left[C_{w1}f_w - \frac{C_{b1}}{\kappa^2} f_{t2} \right] \left(\frac{\tilde{\nu}}{d}^2\right) \\ + \frac{1}{\sigma} \left[\frac{\partial}{\partial x_i} \left( \left(\nu+\tilde{\nu} \right) \frac{\partial \tilde{\nu}}{\partial x_i}\right) +C_{b2} \frac{\partial \tilde{\nu}}{\partial x_j}\frac{\partial \tilde{\nu}}{\partial x_j} \right]
\label{eq:SA}
\end{multline}

From Equation~\ref{eq:SA} we can compute the eddy viscosity from $\tilde{\nu}$ as $\nu_t = \tilde{\nu} f_{v1}$. These equations represent the most popular implementation of the Spalart-Allmaras model.
The terms $f_{v1}$, $\tilde{S}$, and $f_{t2}$ are model-specific 
and contain, for instance, first order flow features (magnitude of the vorticity). 
$C_{b1}$, $C_{w1}$, $C_{b2}$, $\kappa$, and $\sigma$ are constants specific to the model, 
found experimentally. $d$ is the closest distance to a solid surface. 
The first original reference of the model details 
the equations and the values of these constants~\cite{SpalartAllmaras}.


